Transformers for prompt-level EMA non-response prediction

Ecological Momentary Assessments (EMAs) are an important psychological data source for measuring current cognitive states, affect, behavior, and environmental factors from participants in mobile health (mHealth) studies and treatment programs. Non-response, in which participants fail to respond to EMA prompts, is an endemic problem. The ability to accurately predict non-response could be utilized to improve EMA delivery and develop compliance interventions. Prior work has explored classical machine learning models for predicting non-response. However, as increasingly large EMA datasets become available, there is the potential to leverage deep learning models that have been effective in other fields. Recently, transformer models have shown state-of-the-art performance in NLP and other domains. This work is the first to explore the use of transformers for EMA data analysis. We address three key questions in applying transformers to EMA data: 1. Input representation, 2. encoding temporal information, 3. utility of pre-training on improving downstream prediction task performance. The transformer model achieves a non-response prediction AUC of 0.77 and is significantly better than classical ML and LSTM-based deep learning models. We will make our a predictive model trained on a corpus of 40K EMA samples freely-available to the research community, in order to facilitate the development of future transformer-based EMA analysis works.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> sections/copy_abstract.tex <==
\begin{abstract}

Ecological Momentary Assessments (EMAs) are an important psychological data source that can measure the current cognitive states, affect, behavior, and other factors from participants in mobile health (mHealth) studies and treatment programs. However, EMAs suffer from low response rates. {Non-response to EMAs can result from two factors: 1) The participant not being available to respond, 2) The participant not responding despite the EMA being prompted when they are available. We call this specifically as non-compliance, which largely depends on subtle factors such as the participant's interest in the study, emotions, etc. Prior works on EMA non-response lack the ability to separate unavailability from non-compliance and hence only study overall non-response. It is important to address non-compliance in order to improve response rates.
% There have been several prior works on improving response rates by targeting the first factor. These include works that predict non-response based on contextual factors, and these findings can be used to design better EMA delivery systems that deliver EMAs when the participant is likely to respond. However, despite using advanced/intelligent EMA notification systems, we see that a substantial portion of EMA prompts are still unanswered. These can be attributed to the second factor (non-compliance). 
This is the first paper to specifically address the problem of non-compliance. Our work is enabled by a unique study design in which an \textit{on-line availability model was integrated into the EMA delivery system}. This enables us to isolate instances of non-compliance, analyze factors influencing it and predict future non-compliance. The goal of this paper is to lay the foundation for improving compliance, by predicting instances when a participant is at a risk of non-compliance and delivering appropriate compliance interventions.} 
This requires accurate predictions of prompt level EMA compliance that are interpretable enough to inform compliance interventions. {In this paper, 
we model sequences of EMA responses and contextual factors to predict compliance to the next EMA prompt. We analyze the performance of different predictive models, from classical machine learning models to deep models such as bidirectional LSTMs. We find that the latter significantly outperform standard models such as logistic regression, achieving an AUC score of 0.76 on a smoking cessation field study dataset. For the purpose of interpretability, we use an attention layer directly following the input features in the LSTM model. However, we find that the attention weights on the features have high variance due to small sample sizes, making interpretation difficult. We perform $\ell_2$ regularization on the attention layer parameters to achieve stability in interpretation across different subsets of participants, without affecting the performance of the model. We validate our findings about feature importance from the attention layer through feature ablation experiments and statistical analysis. We find that the history of compliance, and emotion items have high feature importance, and location and proximity features have a low feature importance. 


}












\end{abstract}

==> sections/previous_intro.tex <==
\section{introduction (previous)}
Mobile health (mHealth) holds promise for helping improve a wide range of health behaviors, including smoking cessation \cite{riley2011health}, physical activity \cite{klasnja2019efficacy}, stress management \cite{mayor2015mobile} and medication adherence \cite{park2019mobile}.  However a fundamental challenge of mHealth is poor engagement.  It manifests as a slow but steady decline in participation and the use of wearable devices, following an initial period of adoption. Disengagement is highly problematic because it can prevent mHealth technology from improving health outcomes, and it is poorly understood and under-studied.  Three concepts that are sometimes used to define engagement and disengagement are adherence, attrition, and compliance.  Adherence involves following a plan to improve health, such as an exercise, diet, or medication plan \cite{park2019mobile,zhou2019applying}.  Attrition refers to ceasing use of the mHealth app: in clinical trials it is called loss to follow up or dropout \cite{druce2019maximizing}.  Compliance involves responding to a specific request to complete a task or behavior.  If compliance involves repeatedly responding, then it becomes a subset of adherence.\textcolor{red}{does that imply that we know something about the other things in this paragraph?  One possibility: compliance is a proxy for engagement.  Do we believe that?  How do these link to engagement?  Is engagement something that can't be defined, these three things are proxies for the construct of engagement.  Is compliance a different thing?  Conversation early on with Billie: had ubicomp slow but steady decline.  Person who gave more data more valuable, even if they dropped out.  There's all this work on engagement, maybe that's wrong.  Maybe compliance is more important.  Just knowing when they're willing to provide data, also willing to have intervention, may be more valuable than knowing about engagement.  Might be a better strategy to say: people study engagement a lot, compliance less studied, it's very important.  Compliance very different in temporal behavior from engagement.  Engagement has fast decay, compliance has different temporal evolution.  Ubicomp people have already studied engagement, they need to study compliance.  Difference from engagement is a strength.  What is engagement?  Behavioral.  Emotional: actual emotion items.  Cognitive: are they paying attention to what they're doing?}

\begin{itemize}
    \item First talk about compliance.  Why it's important.
    \item Ideal first paragraph? after reading it you know what authors are doing, why it's better.  Like a mini abstract that positions paper.  What is it doing? How does it relate to previous things? Why novel/different?
    \item EMAs are burdensome and people often don't want to do them.  Compliance the thing you need to get EMA.  If you're willing to provide EMA, know possible times when you could intervene.
    \item First to study this properly.
    \item Next paragraph: people have talked about engagement, this is different. Describe figures.
    \item Do we want to cite paper, or refer to figure in another paper?
\end{itemize}

Within mHealth, an important data collection tool is ecological momentary assessments (EMAs)\cite{shiffman2008ecological}.  These involve smartphone applications where either the user initiates a survey, or responds to a prompt containing the EMA and enters survey responses. 
% \textcolor{red}{Stephanie: "... or responds to a prompt containing the EMA."  ---> if you word it like this it might be okay to talk about it as you have. I'm concerned because in intervention science prompts are usually the intervention prompts, not the EMAs. SO you need to be very careful to specify that the PROMPTS you are talking about here only contain the EMA message - they are just EMA message prompts, not "intervention prompts"} 
Generally, EMA prompts are made several times a day over the duration of a study.  Survey questions can include affect,
% \textcolor{red}{Stephanie: say "affect" instead of mood -- mood means something specific and we collected emotions not moods}
environment, and behavioral questions, and thus EMAs can be used to describe how emotions, environmental context, and behavior evolve over time.  They are potentially less subject to recall bias than retrospective surveys, and may generalize better to the real world than laboratory studies \cite{jones2019compliance}.  For instance, \cite{monk2015have} noted that retrospective accounts may underestimate alcohol consumption when compared to in the moment EMAs. However, EMAs are vulnerable to low compliance rates, where compliance refers to the ‘percentage of signal contingent assessments that were responded to in line with the experimental protocol.’ \cite{jones2019compliance} This is mainly due to systematic non-compliance.  For example, a period of high stress may lead to failure to complete an EMA.  In \cite{shiffman2009ecological} they noted compliance of between 50-90\%, while pooling over 126 studies, \cite{jones2019compliance} noted a mean compliance of 75\%.

Low EMA compliance is problematic for three reasons.  Firstly, it reduces statistical power.  Consider the setting where we have a depression drug and we want to use EMA responses
% \textcolor{red}{Stephanie: "EMA responses"} 
to determine if there is a significantly different mean trend in the treatment group vs a control group over the course of the study.  Having more observations within subjects would improve estimates of the difference between mean trends across the two groups.  A second issue is bias: if the non-compliance is systematic, it is likely missing not at random (MNAR), which can introduce bias.  For instance, if someone is upset and thus doesn't respond to a prompt, then their observed responses will tend to be biased towards high positive affect.  A third issue is that in order to deliver appropriate interventions, one would like a clear picture of a user's recent emotions, environment, and behaviors.  However as the time since the last EMA grows, this picture becomes less clear.
% \textcolor{red}{Stephanie: useful to what?}. 
In \cite{jones2019compliance} they discuss the first two of these issues in more detail.

One way to address non-compliance is to determine when a user is prone to \textit{prompt-level EMA non-compliance}, and then intervene.  Prompt-level EMA non-compliance refers to whether or not a user completes a specific EMA prompt.  While it has been studied extensively in the inference setting, where important covariates are identified and hypothesis testing is done to see if they have a significant effect \cite{sokolovsky2014factors,courvoisier2012compliance,turner2017race}, identifying \textit{when} a user is likely not to comply with an EMA given their previous history of compliance and responses is a problem of forecasting with time-varying covariates, which has not been studied yet in this setting.  We thus have three challenges: we first need to frame the forecasting problem for EMA compliance, next we need the forecasts to be good enough to be useful, and finally one needs model interpretability in order to choose an appropriate strategy to increase compliance.
% \textcolor{red}{Stephanie: perhaps say, "...in order to choose an appropriate strategy to increase compliance"}.  
Further, because EMA datasets are relatively small, the model parameters should have sufficiently low variance so that the interpretation is stable even for small datasets.  Particularly, interpretation should be similar when a model is trained across different folds or bootstrap samples.

In this paper, we propose using a bi-directional LSTM architecture with an attention layer directly following the input layer.  This extends \cite{kaji2019attention} to the setting of prompt level EMA
% \textcolor{red}{Stephanie: replace prompt-level with "EMA"} 
compliance.  However, because of our small dataset, we find that the weights of the attention layer and thus the attention activations are not stable across folds of cross validation when applying this method directly.  We evaluate different regularization schemes and find an $\ell_2$ regularization that stabilizes attention activations.  We show that using this model, we achieve an AUC of 0.75 for predicting prompt-level compliance on a recent smoking cessation dataset.

This paper makes three primary contributions: 1) we frame a forecasting problem for prompt-level EMA compliance using time-varying covariates 2) we apply both classical methods and neural networks to this problem, showing that the latter tends to outperform the former 3) we extend a recent interpretable LSTM model to the small data setting via $\ell_2$ regularization.
\begin{itemize}
    \item Have other people solved this problem?
    \item Why is our method better?
    \item Many people have studied item level EMA compliance
    \item They're not interested in what we're interested in
    \item They're not interested in forecasting/prediction
\end{itemize}

Overall
\begin{itemize}
    \item Arg 1: compliance interesting on its own, related to engagement but not the same
    \item Arg 2: no one has looked 
    \item Arg 3: one novel aspect of methodology is use of deep learning, we're only first for compliance forecasting
\end{itemize}

Three paragraphs:
1.  Importance of compliance.  Linked to engagement.  Engagement and compliance are quite different.
2.  Nobody really did compliance before.
3.  Not the first to use deep models but we're the first to use in this way for this setting.

One strategy for intros:
-can write an abstraction: for every paragraph, write a sentence.

Write paragraph.  Take it, rewrite it as an individual sentence.  Then you have a list of sentences, look at those.  Then look at those.  What should the sentences look like?  Don't just give up on the intro being hard.  What do you do when you get stuck?  Rewrite every paragraph as a sentence.

==> sections/temp.tex <==
\section{introduction}
Mobile health (mHealth) technology is a promising tool for health behavior change and maintenance with a broad array of applications, including smoking cessation \cite{riley2011health}, physical activity \cite{klasnja2019efficacy}, stress management \cite{mayor2015mobile} and medication adherence \cite{park2019mobile}. mHealth provides key insights into the contextual and behavioral factors that influence health outcomes, through the ability to collect data from participants in real-time in the field environment. A particularly valuable source of data comes from ecological momentary assessments (EMAs), in which participants answer questions about their mental state, behaviors, and other factors by completing questionnaires, typically multiple times per day. EMA data can be used to assess the risk of adverse behaviors, trigger interventions, or estimate treatment effects. However, a major challenge in EMA data collection 
% is  \emph{prompt level non-compliance}, which 
arises when users fail to complete a survey when prompted {(Non-response). Prior assessments have conflated two factors which combine to produce the overall non-response: 1) Non-availability of the participant. For example, a participant may not be able to respond to an EMA while driving. 2) Non-compliance with the EMA prompt. This is when a participant is available, but fails to respond to an EMA prompt.\footnote{We distinguish between non-compliance and lack of availability, as participants have a `do not disturb' option in our study where they may postpone an EMA if a prompt is triggered while they are occupied with another task.} The distinction between instances of non-compliance and non-availability involves identifying the cause and context of non-response. In this work, the study is designed to check for a participant's availability before triggering an EMA prompt. We leverage the strength of our dataset to isolate instances of non-compliance. Since the participants were always deemed available when an EMA was triggered, every missed instance is treated as non-compliance. Figure \ref{fig:non_response} illustrates the distinction between the two factors: non-response due to non-availability, and due to non-compliance. However, the process of availability detection is not perfect and this is a threat to the validity of our findings. We acknowledge that this work can be further improved with a better availability detection process. We further discuss this in Section \ref{sec:limitations}

Non-response to EMA is problematic for three reasons. First, it reduces the statistical power when testing hypotheses using mHealth data. A second issue is bias: If the non-response is systematic, then it is likely missing not at random (MNAR), a form of bias which is difficult to correct for. A third issue is that in order to deliver appropriate interventions, one would like a clear picture of a user's recent emotions, environment, and behaviors. As the time since the last EMA grows, this picture becomes less clear. 

Prior work has attempted to identify the factors that cause non-response (which they also term as adherence, compliance, engagement) to EMA  \cite{sokolovsky2014factors,courvoisier2012compliance,turner2017race,ono2019affects}. There have also been some recent efforts on predicting EMA non-response using contextual factors such as location, activity, etc. \cite{boukhechba2018contextual} \cite{mishra2017investigating}. The strategies proposed to improve response rates in these works include determining availability and scheduling the EMA prompts accordingly. One common factor among all these prior work is that the EMAs were triggered either based on a pre-determined schedule, or at random through the day. Hence the findings from these studies reflect on the overall non-response, and not compliance. A related area of research is the field of interruptibility and intelligent notification systems \cite{mehrotra2017intelligent,ho2017emu,ho2020quick}. The goal here is to design systems that determine instances suitable for delivering an interruption/notification. The above works use temporal and contextual factors to determine opportune moments when a notification can be delivered. Overall, there have been efforts to improve EMA response rates by improving EMA delivery/notification systems. We specifically address the problem of forecasting non-compliance, which are instances when participants do not respond to EMAs despite using these advanced EMA delivery systems. This is the first, and a key step in enabling compliance interventions. The distinction from prior work is illustrated in Figure \ref{fig:non_response}.

A promising strategy to target the issue of non-compliance is to deliver interventions to improve compliance when the risk of non-compliance is predicted to be high. Several works have developed such interventions for the related task of medication non-compliance \cite{roter1998effectiveness,haynes1987critical}. The goal of this paper is to lay the foundation for similar approaches to improving EMA compliance, by developing a machine learning model for non-compliance, which can accurately predict the risk that a participant will fail to complete the next EMA that they receive.
} 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.45]{figures/non_response2.png}
    \caption{Prior work has addressed the issue of overall non-response (red circle). The cause of non-response could be non-availability, or non-compliance. We are specifically analyzing non-compliance: instances when the participant is available, but fails to respond (shown here in the intersection). When a participant is unavailable (e.g., driving, phone battery low, etc.), they are \textit{unable} to respond. When participants are non-compliant, they are \textit{unwilling} to respond. We believe that separating our non-compliance from overall non-response and predicting these instances is valuable since we can then target compliance interventions.}
    \label{fig:non_response}
\end{figure}

We now describe another related concept, which is disengagement. EMA non-compliance is related to the concept of participant disengagement, which manifests as a decline over time in the participation of a user in a study or treatment program. Several previous works have investigated participant disengagement during mHealth studies~\cite{clawson2015no,lazar2015we}. The end result of disengagement is often attrition, where participants leave the study, also known as loss to follow-up~\cite{druce2019maximizing}. While both disengagement and non-compliance impact the data that can be collected from participants in an mHealth study, they are distinct processes. Non-compliant participants continue to use mHealth devices and apps, but fail to comply with a significant number of requests. In contrast, disengagement manifests as a trend of diminishing participation over time. This distinction is illustrated in Figure \ref{fig:eng_vs_comp}a), which plots disengagement as measured by attrition from early Apple ResearchKit studies \cite{dorsey2017}. Figure~\ref{fig:eng_vs_comp}b)(i) plots the prompt-level compliance from a recent smoking cessation study pooled across users along with a Loess smoother to describe trend.  The disengagement plot shows approximately exponential decay in the number of users as a function of time in the study, while the prompt-level compliance plot has an approximately constant trend. (ii) plots the prompt-level compliance shown for 4 participants in the study. This plot describes the variability in compliance among users (while the average trend is constant).


%%Participant disengagement is a related challenge for mHealth technology
%%While  EMA compliance has received relatively little attention from the mobile health community, there have been significant investigations into the related concept of participant disengagement. Disengagement manifests as a decline in participation of users of wearable devices and/or EMA apps, following an initial period of adoption \cite{clawson2015no,lazar2015we}. While both disengagement and non-compliance limit data collected, these two concepts are distinct.  Disengagement is commonly equated with attrition, where users cease using the mHealth app/device.  This is also called loss to follow up or dropout in clinical trials \cite{druce2019maximizing}. Non-compliance describes users who still continue to use the mHealth app/device, but fail to comply with specific requests. Figure \ref{fig:eng_vs_comp}a) plots disengagement as measured by attrition from early Apple ResearchKit studies \cite{dorsey2017}, while \ref{fig:eng_vs_comp}b) plots the prompt-level compliance from a recent smoking cessation study pooled across users along with a Loess smoother to describe trend.  The disengagement plot shows approximately exponential decay in the number of users as a function of time in the study, while the prompt-level compliance plot has an approximately constant trend.

%%A related concept, which also leads to limitations in data collected, is disengagement.  Disengagement manifests as a decline in participation of users of wearable devices and/or EMA apps, following an initial period of adoption \cite{clawson2015no,lazar2015we}. While both disengagement and non-compliance limit data collected, these two concepts are distinct.  Disengagement is commonly equated with attrition, where users cease using the mHealth app/device.  This is also called loss to follow up or dropout in clinical trials \cite{druce2019maximizing}. Non-compliance describes users who still continue to use the mHealth app/device, but fail to comply with specific requests. Figure \ref{fig:eng_vs_comp}a) plots disengagement as measured by attrition from early Apple ResearchKit studies \cite{dorsey2017}, while \ref{fig:eng_vs_comp}b) plots the prompt-level compliance from a recent smoking cessation study pooled across users along with a Loess smoother to describe trend.  The disengagement plot shows approximately exponential decay in the number of users as a function of time in the study, while the prompt-level compliance plot has an approximately constant trend.

%% There is a substantial body of work using classical machine learning techniques for prediction tasks using EMA data
%%\cite{spanakis2016enhancing}, \cite{saha2017inferring,livingston2017ecological} and \cite{kim2019depression,van2020predicting}

An important characteristic of any solution to the compliance problem is interpretability, which is useful for two reasons. The first is that it provides evidence about whether the model is capturing meaningful relationships in the data. The second is the possibility of using interpretable model weights to identify specific risk factors in order to deliver a targeted compliance intervention. Based on this, our model for predicting EMA completion uses an attention-based deep learning (DL) architecture in order to exploit feature learning while retaining interpretablity. While deep learning approaches have been used successfully for other mHealth data types, such as accelerometry \cite{chen2015deep,10.1145/2733373.2806333,ronao2016human,yang2015deep}, there have been only a few works that use DL to analyze EMA data~\cite{suhara2017deepmood, mikus2018predicting}. We analyze the performance of a bidirectional LSTM model with an attention layer directly following the input. We extend the model proposed in \cite{kaji2019attention} to our setting of prompt level compliance. However, they applied their model to MIMIC III, which has 53,423 hospital admissions.  Our EMA dataset has a much smaller sample size but is still very heterogeneous, and we find that the attention model is unstable across participant samples. We impose regularization constraints on the attention layer in order to stabilize the interpretable feature weights. This model achieves an AUC of 0.76 for predicting prompt level EMA compliance on a real-world dataset of 255 participants from a smoking cessation study. {By analyzing the attention layer weights learned, we see that the location of a participant, and other contextual factors related to the location and time spent at a location have a low attention value (feature importance weight). We verify these findings by performing statistical tests to determine if the compliance rate is significantly different in different locations and find that the difference is not significant. Prior work on predicting non-response report that contextual factors affect the rate of non-response to EMAs \cite{boukhechba2018contextual,mishra2017investigating}. The findings in our study suggest that non-compliance is a phenomenon influenced by internal factors such as emotions, and not  contextual factors such as location. }

In summary, this paper makes the following contributions: 1) we are the first to address the forecasting problem for prompt level EMA compliance (as opposed to overall non-response to EMA). The features used include EMA responses (affect,smoking urge), contextual factors (location, proximity), and time, 2) we develop models with both hand-engineered and deep learned features for this task, finding that the latter give significantly better performance, 3) we extend recent work \cite{kaji2019attention} on interpretable LSTM models, finding that they have very high variance across participant subsets in the small data setting.  We attempt to stabilize the attention weights by regularization, and 4) we visualize and interpret the attention weights learned. We find that the contextual factors such as location have a low attention score (feature importance weight), while features such as the history of compliance, affect, etc. have a high attention score. These findings can assist in designing compliance interventions (when there is a variance in positive/negative emotions, etc.).  

% Our paper is the first effort to forecast prompt level EMA compliance. We use some of the modern deep learning models such as LSTM, which have shown promising performance in other fields and only recently been used in the mHealth domain \cite{suhara2017deepmood,mikus2018predicting}. An additional novelty of our model is that we extend the attention mechanism used for interpretability in a clinical data setting \cite{kaji2019attention} to give us interpretability in the mHealth setting, which proves challenging due to the small amount of data present. 



% \begin{itemize}
%     \item Related concept is engagement: another way to not obtain data needed
%     \item These two concepts are in fact distinct (point out figures)
%     \item Engagement has exponential decay trend, compliance doesn't change much over time.
% \end{itemize}
% Mobile health (mHealth) holds promise for helping improve a variety of health behaviors, including smoking cessation \cite{riley2011health}, physical activity \cite{klasnja2019efficacy}, stress management \cite{mayor2015mobile} and medication adherence \cite{park2019mobile}. Two important components of mHealth include 1) monitoring the environment, physiological, psychological state of participants\textcolor{red}{ there is more to the story than monitoring. We also aim to describe evolution.} and 2) delivering Just-in-Time Interventions \cite{liao2018just,jaimes2014stress,nahum2018just}\textcolor{red}{ I don't think that JITAI is important enough to be this early.  Before a JITAI we need to collect information and we can't even do that well with compliance/engagement issues.  I think it could be something like collecting data and then using it}. This requires the user to provide information through surveys or prompts, and perform the intervention tasks specified. However, low participant engagement and compliance is a key challenge to the success of mHealth \cite{druce2019maximizing}. Compliance in mHealth involves response to a specific request to complete a task or behavior. A related concept used is that of engagement and disengagement of users. Disengagement of users manifests as a slow but steady decline in participation of users of wearable devices, following an initial period of adoption \cite{clawson2015no,lazar2015we}. Disengagement and non-compliance are related concepts which result in a reduction in the amount of data provided by the user. However, there are differences between the two concepts. Disengagement is commonly used to describe participants who cease using the mHealth app/device, also called loss to follow up or dropout in clinical trials \cite{druce2019maximizing}. Non-compliance on the other hand is the behavior of participants who still continue to use the mHealth app/device or be part of the study, but fail to comply with the requested task at certain tasks. While disengagement has been identified as a challenge and studied in the case of mHealth devices \cite{clawson2015no,lazar2015we}, there has been relatively lesser work in the mHealth space on compliance. \cite{sokolovsky2014factors,courvoisier2012compliance,turner2017race} identify low compliance as an issue and perform preliminary analysis on the factors influencing compliance. In this paper, we focus on the compliance of users to Ecological Momentary Assessment (EMA) prompts. EMA prompts are an important data collection tool used in mHealth \cite{shiffman2008ecological}. They contain survey questions about affect, environment, and behavior of users. Our paper is the first effort to forecast prompt level EMA compliance. We use some of the modern deep learning models such as LSTM, which have shown promising performance in other fields and only recently been used in the mHealth domain \cite{suhara2017deepmood,mikus2018predicting}. An additional novelty of our model is that we extend the attention mechanism used for interpretability in a clinical data setting \cite{kaji2019attention} to give us interpretability in the mHealth setting, which proves challenging due to the small amount of data present. 

\begin{figure}
        \centering
        \begin{subfigure}{.5\textwidth}
          \centering
          \includegraphics[scale=0.22]{figures/engagement.png}
    
          \caption{}
          \label{fig:eng}
        \end{subfigure}%
        \begin{subfigure}{.5\textwidth}
          \centering
          \includegraphics[scale=0.22]{figures/compliance_subject.png}
          \caption{}
          \label{fig:comp}
        \end{subfigure}
        \caption{Trend of disengagement vs compliance of participants (a) Percentage of daily users in the first five smartphone research apps developed by ResearchKit (March 09 to October 05, 2015). [Figure adapted from \cite{dorsey2017} used without permission.] (b)(i) Pooled prompt level EMA compliance over two weeks in a smoking cessation study. Compliance has approximately a constant trend (quite different from the disengagement trend observed in (a)). (ii) Prompt level compliance shown for 4 participants. There is substantial heterogeneity in compliance trajectories between participants.
    }
        \label{fig:eng_vs_comp}
    \end{figure}
    
% The difference between the concept of engagement and compliance is illustrated in Figure \ref{fig:eng_vs_comp}. Figure \ref{fig:eng} is a visualization of the percentage of daily users in five smartphone research apps. These apps were developed by ResearchKit, an open source platform for smartphone apps for health research by Apple. This analysis was performed by the authors in \cite{dorsey2017}, determining the use of smartphone apps in health research. Figure \ref{fig:eng} has been obtained from \cite{dorsey2017} and used without permission. Figure \ref{fig:comp} is a plot of the prompt level EMA compliance of participants in a smoking cessation study we consider in this paper. The compliance is a binary variable, with a value of 1 when the user completed an EMA prompt and 0 otherwise. The red line indicates the locally estimated scatterplot smoothing (loess) plot over the two week horizon, giving us an estimate of the compliance of users. From this figure, we see that while engagement and compliance are related, they have certain differences. There has been previous work in the mHealth space identifying the challenges posed by disengagement. \cite{clawson2015no,lazar2015we} have studied the factors influencing users to disengage from wearable healthcare devices and smart devices. However, the problem of compliance is less studied in the mHealth community. Low EMA compliance is problematic for three reasons.  Firstly, it reduces statistical power.  Consider the setting where we have a depression drug and we want to use EMA responses to determine if there is a significantly different mean trend in the treatment group vs a control group over the course of the study.  Having more observations within subjects would improve estimates of the difference between mean trends across the two groups.  A second issue is bias: if the non-compliance is systematic, it is likely missing not at random (MNAR), which can introduce bias.  For instance, if someone is upset and thus doesn't respond to a prompt, then their observed responses will tend to be biased towards high positive affect.  A third issue is that in order to deliver appropriate interventions, one would like a clear picture of a user's recent emotions, environment, and behaviors.  However as the time since the last EMA grows, this picture becomes less clear. In \cite{jones2019compliance} they discuss the first two of these issues in more detail. There have been a lot of works focusing on statistical inference on the factors influencing prompt level compliance \cite{sokolovsky2014factors,courvoisier2012compliance,turner2017race,ono2019affects}. However, there is no existing work on forecasting prompt level compliance to EMA. Forecasting prompt level compliance is useful since one way to address non-compliance is to determine when a user is prone to \textit{prompt-level EMA non-compliance}, and then intervene.  

% There has been a lot of previous work using classical machine learning techniques on data derived from EMAs \cite{saha2017inferring,livingston2017ecological}\textcolor{red}{cite some more}. However, there are very few recent works \cite{suhara2017deepmood,mikus2018predicting} leveraging deep learning models, which have shown good performance in other domains. In this paper, we propose a bidirectional LSTM model with an attention layer directly following the input. We extend the model proposed in \cite{kaji2019attention} to our setting of prompt level compliance. However, due to the small data size and heterogeneity in the data, we find that the attnetion model is unstable across participant samples. We impose regularization constraints on the attention layer, to stabilize the interpretable feature weights. This model achieves an AUC of 0.75 for predicting prompt level EMA compliance on a recent smoking dataset. 

% This paper makes three primary contributions: 1) We frame a forecasting problem for prompt level EMA compliance using time-varying covariates 2) We apply both classical machine learning and deep learning methods to this problem and demonstrate that the latter outperforms the former 3) We extend a recent interpretability technique proposed in a clinical setting to our setting where we have smaller amount of data. 
